Rediscover Climate Change during Global Warming Slowdown via Wasserstein Stability Analysis

Climate change is one of the key topics in climate science. However, previous research has predominantly concentrated on changes in mean values, and few research examines changes in Probability Distribution Function (PDF). In this study, a novel method called Wasserstein Stability Analysis (WSA) is developed to identify PDF changes, especially the extreme event shift and non-linear physical value constraint variation in climate change. WSA is applied to 21st-century warming slowdown period and is compared with traditional mean-value trend analysis. The result indicates that despite no significant trend, the central-eastern Pacific experienced a decline in hot extremes and an increase in cold extremes, indicating a La Nina-like temperature shift. Further analysis at two Arctic locations suggests sea ice severely restricts the hot extremes of surface air temperature. This impact is diminishing as sea ice melts. Overall, based on detecting PDF changes, WSA is a useful method for re-discovering climate change.

==> Results.tex <==
During 1998 - 2012 period, global mean surface temperature experienced a slower increase, which is referred to as "global warming hiatus" in early studies \cite{Modak2021,Douville2015,Kosaka2013,Lee2015,Delworth2015,England2014,Li2015}. 
Recent research indicated that there was no true "hiatus" during that time, but the global surface temperatures were still rising, albeit more slowly \cite{Simmons2017}. 
This phenomenon suggests that physical processes other than the anthropogenic warming trend play a role in climate change, and the detection of PDF change may provide us with new information for this period.  
Therefore, by comparing the performance of WSA with traditional trend analysis, we can evaluate the similarity and difference between these two approaches, which could advance our understanding of climate science and inform future research in this area.

Figure \ref{fig:wdis_trend}a depicts the Wasserstein distance between SAT PDFs during 1998-2005 and 2005-2012. 
There are two main large-scale significant W-distance signals appearing in Figure \ref{fig:wdis_trend}a: the central eastern Pacific and the Barents-Kara Sea. 
The central eastern Pacific has the greatest W-distance, with values ranging from 0.08 to 0.24; nevertheless, there is no discernible trend (Figure \ref{fig:wdis_trend}b). 
Another noticeable W-distance signal could be seen over the Barents-Kara Sea, which is located inside a significant warming trend zone in the Arctic (Figure \ref{fig:wdis_trend}b). 
The following analysis will mainly focus on signals over central eastern Pacific and Barents-Kara Sea to highlight the information that W-distance can provide about climate change. 
In practice, we found that due to the presence of sea ice, the surface temperature distribution shows a large discontinuous in the Arctic region.
As a result, the areal average in this region may smash some information from individual grids. 
To avoid this, we selected three special sites to do further PDF analysis: \\
1. Site A (90 $^o$W, 0): one site with a significant W-distance signal but without a significant linear trend; \\
2. Sites B (66 $^o$E,79 $^o$N) and C (131 $^o$E,79 $^o$N): both sites exhibit significant linear trends. However, Site B has a significant W-distance while C does not. 


Figure \ref{fig:siteA} shows the SAT PDFs and their changes from the 1998-2005 period to the 2005-2013 period at Site A. 
The mean value and standard deviation stay relatively stable within the 1998-2005 and 2005-2013 periods. 
However, in the second period, the hot extremes (more than two standard deviations, 25 $^o$C) decrease by more than ten days per year, while the mild hot events (near one standard deviation) increase by roughly 30 days per year. 
Meanwhile, the cold extremes (less than -2 standard deviations, 19 $^o$C) increase by more than ten days per year, while the mild cold events (near -1 standard deviation) decrease by more than 30 days per year. 
The hot extreme decreasing and cold extreme increasing indicate a La Nina-like SAT shift. 
Many recent studies argue that the 21st slowdown period is in the negative phase of Pacific Decadal Oscillation, and this strong low-frequency variability canceled out some parts of the global warming trend
\cite{Douville2015,Kosaka2013,Lee2015,England2014}. 
Our W-distance result agrees well with this conclusion and extends the results from the perspective of PDF change. 
Indeed, even though the mean value does not show a significant trend, we can still observe the La Nina-like SAT shift from extreme event change, which is reflected by the strong PDF change and the corresponding significant W-distance. 


Site B is another region with a significant W-distance, suggesting a strong PDF change from the 1998-2005 period to the 2005-2013 period (Figure \ref{fig:siteBC} (a) and (c)). 
At Site B, SAT shows significant warming from -10.2 $^o$C to -6.4 $^o$C. 
Meanwhile, the standard deviation decreases from 9.9 $^o$C to 7.4 $^o$C, indicating an elimination of SAT variation. 
Since Site B is located within a zone covered by sea ice, the maximum SAT is strongly constrained to being near the frozen line in both periods, and thus this causes a sharp frequency jump near the frozen line (Figure \ref{fig:siteBC} (a)). 
However, as the mean value increases and the standard deviation decreases during the second period, the frozen line at Site B shifts significantly to the left.
As a result, the frequency peak of hot events shifts to the left. 
Meanwhile, the slope near the frozen line becomes flatter, leading to a smoother PDF shape. 
In contrast, Site C exhibits a change that follows a similar pattern but is considerably smaller in extent in terms of mean value, standard deviation, and frozen line shift (Figure \ref{fig:siteBC} (b) and (d)). 
Consequently, W-distance at Site C is smaller than that at Site B and fails the 99\% significant test. 
Actually, the existence of sea ice strongly limits the maximum surface temperature and the corresponding surface air temperature near the frozen line. 
Therefore, the sharp peak shape of SAT PDF appears in regions covered by sea ice. 
Nevertheless, regions with normal ocean conditions are expected to have a more uniform distribution.
Therefore, the alteration in Site B and Site C suggests that the variability in sea ice concentration may play a role in the SAT PDF change from the first to the second period.

By checking the full-time series in two periods, we can better understand the PDF change at Site B and Site C. 
From 1998-2005 period to 2005-2013 period, the interval with $\pm1$ standard deviation  shrinks and moves upward at Site B because of the change in mean value and standard deviation  (Figure \ref{fig:seaice}(a)). 
Clearly, this change leads to most of the SAT variabilities being below +1 standard deviation and also more cold extremes. 
For Site C, we can see a similar change but in a much smaller magnitude (Figure \ref{fig:seaice} (b)).  
As discussed, this difference can be attributed to the sea ice and its strong temperature constraint. 
Figure \ref{fig:seaice} (c) shows the sea ice concentration change between 1998-2005 and 2005-2013. 
We can see that Site B is in a zone where sea ice is melting the most. Hence the PDF change at Site B is the most intense. 
As a comparison, Site C also experiences a sea ice loss but to a relatively small extent. 
As the temperature increases, the sea ice concentration decreases, and the effect of sea ice restriction gradually fades.  
This is why Site C also displays a similar PDF change but with a less significant level. 
In summary, the significant W-distance change at Site B implies the removal of physical temperature constraint imposed by sea ice that causes the sharp peak near the frozen line in PDF. 


Overall, by detecting changes in the probability density function (PDF) between the early and later periods during slowdown period, results demonstrate the WSA's capability to identify the two physical processes associated with the warming deceleration: the La Nina-like tropical Pacific temperature shift and the sea ice loss-induced PDF transition. 
% The transition of the Pacific Decadal Variability into a negative phase (La Nina-like) is one of the primary causes of this warming deceleration, which partially offsets the anthropogenic warming trend. 
% On the other hand, a recent reevaluation of reanalysis data indicates that the warming trend in Arctic regions was previously underestimated due to issues with surface temperature estimation in regions . (Simmons 2017). 
% 

==> figure/figure.tex <==
\begin{figure}
    \centering
    %\includegraphics[width=15cm]{figure/Figure1.pdf}
    \includegraphics[scale=0.69]{figure/Figure1.pdf}
    \caption{ (a) Wasserstein distance between probability distribution functions during 1998-2005 and 2005-2012. (b) Linear trend during 1998-2012. Only statistically significant regions (99\% for Wasserstein distance and 95\% for linear trend) are shown. Three sites, A (90$^o$W, 0), B (66$^o$E, 79$^o$N), and C (131$^o$E, 79$^o$N), have been chosen for further analysis. }
    \label{fig:wdis_trend}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{figure/hiatus_wtest.eps}
%     \caption{Global mean near-surface temperature possibility distribution function during 1998-2005 and 2006-2013. }
%     \label{fig:wdist_global_mean}
% \end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=15cm]{figure/Figure2.pdf}
    \includegraphics[scale=0.65]{figure/Figure2.pdf}
    \caption{
   (a) Probability distribution functions (PDFs) for the periods 1998–2005 (blue) and 2005–2012 (red).  The bottom tick labels represent observed temperature values from 2005 to 2012, whereas the top tick labels represent observed temperature values from 1998 to 2005. (b) The difference between two PDFs of  normalized temperature series at site A (90$^o$W, 0). The frequency has been normalized as days per year. The mean value for the time period is shown by the blanketed number in the legend.
    }
    \label{fig:siteA}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=15cm]{figure/Figure3.pdf}
    \includegraphics[scale=0.69]{figure/Figure3.pdf}
    \caption{Same as Figure \ref{fig:siteA}. Panel (a) and (c) is for Site B, and Panel (b) and (d) is for Site C. The dashed lines in Panel (a) and (b) represent the ocean frozen temperature (-1.7$^o$C) in two distributions (blue for 1998-2005 and red for 2005-2012). 
    }
    \label{fig:siteBC}
\end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=16cm]{figure/figure4.pdf}
    \includegraphics[scale=0.69]{figure/figure4.pdf}
    \caption{Full daily 2m temperature time series of 1998-2005 (blue) and 2005-2012 (red) at Site B is plotted in Panel (a), and the counterpart at Site C is plotted in Panel (b). Panel (c) shows the sea ice concentration change (unit: \%) between 1998-2005 and 2005-2012.  
    }
    \label{fig:seaice}
\end{figure}

